Precompactness notions in Kaplansky--Hilbert modules and extensions with discrete spectrum

This paper is a continuation of our work on the functional-analytic core of the classical Furstenberg-Zimmer theory. We introduce and study (in the framework of lattice-ordered spaces) the notions of total order-boundedness and uniform total order-boundedness. Either one generalizes the concept of ordinary precompactness known from metric space theory. These new notions are then used to define and characterize "compact extensions" of general measure-preserving systems (with no restrictions on the underlying probability spaces nor on the acting groups). In particular, it is (re)proved that compact extensions and extensions with discrete spectrum are one and the same thing. Finally, we show that under natural hypotheses a subset of a Kaplansky-Banach module is totally order bounded if and only if it is cyclically compact (in the sense of Kusraev).

==> mathcoms.tex <==
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{mymathcoms}


%% 
%% Constants
%% 

% Lowercase mathrm

\newcommand{\ua}{\mathrm{a}}
\newcommand{\ub}{\mathrm{b}}
\newcommand{\uc}{\mathrm{c}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\ue}{\mathrm{e}}
\newcommand{\uf}{\mathrm{f}}
\newcommand{\ug}{\mathrm{g}}
\newcommand{\uh}{\mathrm{h}}
\newcommand{\ui}{\mathrm{i}}
\newcommand{\uj}{\mathrm{j}}
\newcommand{\uk}{\mathrm{k}}
\newcommand{\ul}{\mathrm{l}}
\newcommand{\um}{\mathrm{m}}
\newcommand{\un}{\mathrm{n}}
\newcommand{\uo}{\mathrm{o}}
% The command \up is defined by babel if French is loaded as a language
% But since I only use this French command very rarely, a redefinition 
% doesn't cause much harm.
\AtBeginDocument{
  \ifdefined\up
    \let\frup\up
    \renewcommand{\up}{\mathrm{p}}
  \else 
    \newcommand{\up}{\mathrm{p}}
  \fi
}
\newcommand{\uq}{\mathrm{q}}
\newcommand{\ur}{\mathrm{r}}
\newcommand{\us}{\mathrm{s}}
\newcommand{\ut}{\mathrm{t}}
\newcommand{\uu}{\mathrm{u}}
\newcommand{\uv}{\mathrm{v}}
\newcommand{\uw}{\mathrm{w}}
\newcommand{\ux}{\mathrm{x}}
\newcommand{\uy}{\mathrm{y}}
\newcommand{\uz}{\mathrm{z}}

% Uppercase mathrm

\newcommand{\uA}{\mathrm{A}}
\newcommand{\uB}{\mathrm{B}}
\newcommand{\uC}{\mathrm{C}}
\newcommand{\uD}{\mathrm{D}}
\newcommand{\uE}{\mathrm{E}}
\newcommand{\uF}{\mathrm{F}}
\newcommand{\uG}{\mathrm{G}}
\newcommand{\uH}{\mathrm{H}}
\newcommand{\uI}{\mathrm{I}}
\newcommand{\uJ}{\mathrm{J}}
\newcommand{\uK}{\mathrm{K}}
\newcommand{\uL}{\mathrm{L}}
\newcommand{\uM}{\mathrm{M}}
\newcommand{\uN}{\mathrm{N}}
\newcommand{\uO}{\mathrm{O}}
\newcommand{\uP}{\mathrm{P}}
\newcommand{\uQ}{\mathrm{Q}}
\newcommand{\uR}{\mathrm{R}}
\newcommand{\uS}{\mathrm{S}}
\newcommand{\uT}{\mathrm{T}}
\newcommand{\uU}{\mathrm{U}}
\newcommand{\uV}{\mathrm{V}}
\newcommand{\uW}{\mathrm{W}}
\newcommand{\uX}{\mathrm{X}}
\newcommand{\uY}{\mathrm{Y}}
\newcommand{\uZ}{\mathrm{Z}}

%% 
%% Symbols for fields etc.
%%
\newcommand{\A}{\mathbb{A}} 
\newcommand{\E}{\mathbb{E}} 
\newcommand{\N}{\mathbb{N}} 
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\F}{\mathbb{F}}
\renewcommand{\O}{\mathcal{O}} % Mea culpa, ...
\renewcommand{\P}{\mathbb{P}} % ... mea maxima culpa.

%%
%% Math operators (that are functions)
%%

\newcommand{\co}{\operatorname{co}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\divop}{\operatorname{div}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\esssup}{\operatorname{ess\,sup}}
\newcommand{\essrang}{\operatorname{ess\,rang}}
\newcommand{\ext}{\operatorname{ext}}
\newcommand{\fix}{\operatorname{fix}}
\renewcommand{\gcd}{\operatorname{gcd}} % don't want this to change with the language
\newcommand{\grad}{\operatorname{grad}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\interior}{\operatorname{int}}
\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\lin}{\operatorname{lin}}
\newcommand{\orb}{\operatorname{orb}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\ran}{\operatorname{ran}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\res}{\operatorname{res}}
\newcommand{\rg}{\operatorname{rg}}
\newcommand{\rot}{\operatorname{rot}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\tr}{\operatorname{tr}}

% Interesting: These are not functors or categories, yet capitalized

\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Re}{\operatorname{Re}}

%%
%% Functors
%%

\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Mor}{\operatorname{Mor}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\Iso}{\operatorname{Iso}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Per}{\operatorname{Per}}
\newcommand{\Gal}{\operatorname{Gal}} % \Gal(E/F)
\newcommand{\SL}{\operatorname{SL}} % \SL(n, \R)
\newcommand{\GL}{\operatorname{GL}} % \GL(n, \R)
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Mat}{\operatorname{Mat}} % \Mat(n, m; \R), \Mat_n(\R)
\newcommand{\Bil}{\operatorname{Bil}}

%%
%% Categories
%%

\newcommand{\Fct}{\mathrm{Fct}} % \Fct(\mathcal{C}, \mathcal{D})
\newcommand{\Grp}{\mathbf{Grp}}
\newcommand{\MDS}{\mathbf{MDS}}
\newcommand{\Mod}{\mathbf{Mod}} % \Mod_R
\newcommand{\Ring}{\mathbf{Ring}}
\newcommand{\Set}{\mathbf{Set}}
\newcommand{\TDS}{\mathbf{TDS}}
\newcommand{\Vect}{\mathbf{Vect}} % \Vect(\R), \Vect_n(\R)

\newcommand{\Ob}{\mathrm{Ob}}
\newcommand{\op}{\mathrm{op}}
\newcommand{\from}{\leftarrow}

%% 
%% Measures
%%

\newcommand{\da}{\,\mathrm{d}a}
\newcommand{\db}{\,\mathrm{d}b}
\newcommand{\dc}{\,\mathrm{d}c}
\newcommand{\dd}{\,\mathrm{d}d}
\newcommand{\de}{\,\mathrm{d}e}
\newcommand{\df}{\,\mathrm{d}f}
\newcommand{\dg}{\,\mathrm{d}g}
% \renewcommand{\dh}{\,\mathrm{d}h} % Already defined!
\newcommand{\di}{\,\mathrm{d}i}
% \renewcommand{\dj}{\,\mathrm{d}j} % Already defined!
\newcommand{\dk}{\,\mathrm{d}k}
\newcommand{\dl}{\,\mathrm{d}l}
\newcommand{\dm}{\,\mathrm{d}m}
\newcommand{\dn}{\,\mathrm{d}n}
% \newcommand{\do}{\,\mathrm{d}o} % Already defined!
% \newcommand{\dp}{\,\mathrm{d}p} % Already defined!
% \newcommand{\dq}{\,\mathrm{d}q} % Already defined!
\newcommand{\dr}{\,\mathrm{d}r}
\newcommand{\ds}{\,\mathrm{d}s}
\newcommand{\dt}{\,\mathrm{d}t}
\newcommand{\du}{\,\mathrm{d}u}
\newcommand{\dv}{\,\mathrm{d}v}
\newcommand{\dw}{\,\mathrm{d}w}
\newcommand{\dx}{\,\mathrm{d}x}
\newcommand{\dy}{\,\mathrm{d}y}
\newcommand{\dz}{\,\mathrm{d}z}

\newcommand{\dalpha}{\,\mathrm{d}\alpha}
\newcommand{\dbeta}{\,\mathrm{d}\beta}
\newcommand{\dgamma}{\,\mathrm{d}\gamma}
\newcommand{\ddelta}{\,\mathrm{d}\delta}
\newcommand{\depsilon}{\,\mathrm{d}\epsilon}
\newcommand{\dzeta}{\,\mathrm{d}\zeta}
\newcommand{\deta}{\,\mathrm{d}\eta}
\newcommand{\dtheta}{\,\mathrm{d}\theta}
\newcommand{\diota}{\,\mathrm{d}\iota}
\newcommand{\dkappa}{\,\mathrm{d}\kappa}
\newcommand{\dlambda}{\,\mathrm{d}\lambda}
\newcommand{\dmu}{\,\mathrm{d}\mu}
\newcommand{\dnu}{\,\mathrm{d}\nu}
\newcommand{\dxi}{\,\mathrm{d}\xi}
% No \omikron
\newcommand{\dpi}{\,\mathrm{d}\pi}
\newcommand{\drho}{\,\mathrm{d}\rho}
\newcommand{\dsigma}{\,\mathrm{d}\sigma}
\newcommand{\dtau}{\,\mathrm{d}\tau}
\newcommand{\dupsilon}{\,\mathrm{d}\upsilon}
\newcommand{\dphi}{\,\mathrm{d}\phi}
\newcommand{\dchi}{\,\mathrm{d}\chi}
\newcommand{\dpsi}{\,\mathrm{d}\psi}
\newcommand{\domega}{\,\mathrm{d}\omega}

\newcommand{\dA}{\,\mathrm{d}A}
\newcommand{\dB}{\,\mathrm{d}B}
\newcommand{\dC}{\,\mathrm{d}C}
\newcommand{\dD}{\,\mathrm{d}D}
\newcommand{\dE}{\,\mathrm{d}E}
\newcommand{\dF}{\,\mathrm{d}F}
\newcommand{\dG}{\,\mathrm{d}G}
\newcommand{\dH}{\,\mathrm{d}H}
\newcommand{\dI}{\,\mathrm{d}I}
\newcommand{\dJ}{\,\mathrm{d}J}
\newcommand{\dK}{\,\mathrm{d}K}
\newcommand{\dL}{\,\mathrm{d}L}
\newcommand{\dM}{\,\mathrm{d}M}
\newcommand{\dN}{\,\mathrm{d}N}
\newcommand{\dO}{\,\mathrm{d}O}
\newcommand{\dP}{\,\mathrm{d}P}
\newcommand{\dQ}{\,\mathrm{d}Q}
\newcommand{\dR}{\,\mathrm{d}R}
\newcommand{\dS}{\,\mathrm{d}S}
\newcommand{\dT}{\,\mathrm{d}T}
\newcommand{\dU}{\,\mathrm{d}U}
\newcommand{\dV}{\,\mathrm{d}V}
\newcommand{\dW}{\,\mathrm{d}W}
\newcommand{\dX}{\,\mathrm{d}X}
\newcommand{\dY}{\,\mathrm{d}Y}
\newcommand{\dZ}{\,\mathrm{d}Z}

%%
%% Miscellaneous
%%

%\renewcommand{\1}{\mathbbm{1}}

% Correct quantor spacing

\let\oldforall\forall
\let\oldexists\exists
\renewcommand{\forall}{\,\oldforall\,}
\renewcommand{\exists}{\,\oldexists\,}

% "Geschmackssache.", sagte der Affe und biss in die Seife.

\let\subob\leq
\let\supob\geq
%\renewcommand{\leq}{\leqslant}
%\renewcommand{\geq}{\geqslant}
\newcommand{\oldleq}{\subob}
\newcommand{\oldgeq}{\supob}

% \varepsilon is _way_ cooler than \epsilon.

\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\varepsilon}
\let\oldphi\phi
\renewcommand{\phi}{\varphi}
\let\oldtheta\theta
\renewcommand{\theta}{\vartheta}

% Either use \subseteq or \subsetneq, \subset is not needed and misguiding.

\renewcommand{\subset}{\subseteq}
\renewcommand{\supset}{\supseteq}

% correctly typesets := and =:
\newcommand{\defeq}{\mathrel{\vcentcolon=}}
\newcommand{\eqdef}{\mathrel{=\vcentcolon}}

% Creates a version of \mid that can (only) be used between 
% \left and \right and scales correctly.
\newcommand{\mmid}{\,\middle|\,}

% Left and right ceiling

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Dots for parameters, to be used if f(\cdot) doesn't cut it
\newcommand{\pardot}{\mathbin{\cdot}}

\newcommand{\smallboxtimes}{\mathbin{\XBox}}

\renewcommand{\tilde}[1]{\widetilde{#1}}
\renewcommand{\hat}[1]{\widehat{#1}}

\let\longimplies\implies
\renewcommand{\implies}{\longimplies}

\newcommand{\myqedsymbol}{\ensuremath{\Box}}

% In case a proof doesn't work out as planned (requires tikz)

\newcommand{\semiqed}{
  \parfillskip=0pt\nobreak\hfill
  {
    \scalebox{0.5}{
    \def\sqedlength{0.25}
    \def\sqedlength{0.5}
    \begin{tikzpicture}[overlay]
      \draw[densely dashed](0.0, 0.0) -- (0.0, \sqedlength);
      \draw[densely dashed](0.0, \sqedlength) -- (\sqedlength, \sqedlength);
      \draw[densely dashed](\sqedlength, \sqedlength) -- (\sqedlength, 0.0);
      \draw[densely dashed](0.0, 0.0) -- (\sqedlength, 0.0);
    \end{tikzpicture}
      }
  }\hspace{2px}
  \par
}

\newcounter{proofstep}
\newcommand{\step}[1][]{
  \refstepcounter{proofstep}
  \ifthenelse{\equal{#1}{}}{%
    %omitted 
    \par\textbf{\mystepname\,\theproofstep:}
  }{%supplied
    \par\textbf{\mystepname\,\theproofstep\,{\normalfont(#1)}:}\unskip
  }
}

%%% \vvvert (|||x||| Norm)

\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * matha
      <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
      }{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}
\DeclareFontSubstitution{U}{matha}{m}{n}

% Math symbol font mathb
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}

% Symbol definition
\DeclareMathDelimiter{\vvvert}{0}{matha}{"7E}{mathx}{"17}

